Design of an integrated hybrid plasmonic-photonic device for all-optical switching and reading of spintronic memory

We introduce a novel integrated hybrid plasmonic-photonic device for all-optical switching and reading of nanoscale ferrimagnet bits. The racetrack memory made of synthetic ferrimagnetic material with a perpendicular magnetic anisotropy is coupled on to a photonic waveguide onto the indium phosphide membrane on silicon platform. The device which is composed of a double V-shaped gold plasmonic nanoantenna coupled with a photonic crystal cavity can enable switching and reading of the magnetization state in nanoscale magnetic bits by enhancing the absorbed energy density and polar magneto-optical Kerr effect (PMOKE) locally beyond the diffraction limit. Using a three-dimensional finite-difference time-domain method, we numerically show that our device can switch and read the magnetization state in targeted bits down to ~100 nm in the presence of oppositely magnetized background regions in the racetrack with widths of 30 to 120 nm, clearly outperforming a bare photonic waveguide. Our hybrid device tackles the challenges of nonlinear absorption in the waveguide, weak PMOKE, and size mismatch between spintronics and integrated photonics. Thus, it provides missing link between the integrated photonics and nanoscale spintronics, expediting the development of ultrafast and energy efficient advanced on-chip applications.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


